Direct Monocular Odometry Using Points and Lines

Most visual odometry algorithm for a monocular camera focuses on points, either by feature matching, or direct alignment of pixel intensity, while ignoring a common but important geometry entity: edges. In this paper, we propose an odometry algorithm that combines points and edges to benefit from the advantages of both direct and feature based methods. It works better in texture-less environments and is also more robust to lighting changes and fast motion by increasing the convergence basin. We maintain a depth map for the keyframe then in the tracking part, the camera pose is recovered by minimizing both the photometric error and geometric error to the matched edge in a probabilistic framework. In the mapping part, edge is used to speed up and increase stereo matching accuracy. On various public datasets, our algorithm achieves better or comparable performance than state-of-the-art monocular odometry methods. In some challenging texture-less environments, our algorithm reduces the state estimation error over 50%.

==> analysis.tex <==
In this section, we discuss some details of plane SLAM.





\subsection{Height effects}

Unlike the RGB-D plane SLAM, our plane measurement comes from the pop-up plane whose scale is determined by the camera height in Section \ref{sec:pop_up_pose}. So the SLAM plane measurements themselves cannot constraint the camera height anymore, which can only be constrained by other information such as odometry measurements or other sensors such as IMU. If these information is not accessible, the map scale will drift using the plane SLAM alone.

During all the experiments, we didn't meet the scale drifting problem because the cameras are kept at nearly constant height. If 

During all the experiments, we assume that cameras are kept at nearly a constant height so that our algorithm can keep the global scale.

During the experiments, we assume that the initial camera height to be 1m or using ground truth height in order to get an absolute 3D plane model scale. 

The cameras are kept at nearly a constant height in all the experiments performed above, our algorithm can keep the global scale without drifting.

But if this assumption is violated or relaxed, our \textit{Pop-up plane SLAM} might not keep scale consistency.

%But if this assumption is violated or relaxed, our \textit{Pop-up plane SLAM} might not keep scale consistency.

%During the experiments, we assume that the initial camera height to be 1m or using ground truth height in order to get an absolute 3D plane model scale. 
%The cameras are kept at nearly a constant height in all the experiments performed above, our algorithm can keep the global scale without drifting.





\subsection{sparsification}


\subsection{Limitations and future work}

